Ballpark Learning: Estimating Labels from Rough Group Comparisons

We are interested in estimating individual labels given only coarse, aggregated signal over the data points. In our setting, we receive sets ("bags") of unlabeled instances with constraints on label proportions. We relax the unrealistic assumption of known label proportions, made in previous work; instead, we assume only to have upper and lower bounds, and constraints on bag differences. We motivate the problem, propose an intuitive formulation and algorithm, and apply our methods to real-world scenarios. Across several domains, we show how using only proportion constraints and no labeled examples, we can achieve surprisingly high accuracy. In particular, we demonstrate how to predict income level using rough stereotypes and how to perform sentiment analysis using very little information. We also apply our method to guide exploratory analysis, recovering geographical differences in twitter dialect.

==> experiments.tex <==
In this section we evaluate our algorithm on the two real-world applications of Section \ref{sec:app}.


\subsection{One-Word Text Classification}

%\dnote{ Goal of the experiment (compare ourselves to Greg, see how well we can do with a lot less signal}
In this experiment, we compare ourselves to state-of-the-art methods for text classification using weak signals.

%1. Explain datasets
\xhdr{Data and Tasks}
In order to evaluate our {one-word text classification} algorithm, we prepared the following datasets:

\begin{itemize}
\item{\bf 20 newsgroups } 
The 20 Newsgroups dataset contains approximately 20,000 newsgroup posts across 20 different newsgroups. Some of the newsgroups are closely related (e.g., comp.sys.ibm.pc.hardware and \\ comp.sys.mac.hardware), while others are further apart (rec.sport.hockey and sci.space).
The task is to classify messages according
to the newsgroup to which they were posted. We report our results for the $3$ 
binary subsets ($2000$ instances) used in \cite{Druck08features}: med-space, ibm-mac, and baseball-hockey.
\item {\bf Movie Reviews } The Movie Reviews dataset \cite{PangLee:04a}
contains 1000 positive and 1000 negative movie reviews written before 2002. The task is to classify the sentiment of movie reviews as positive or negative.
\end{itemize}



\xhdr{Baselines}
Under our setting, there are no labeled instances. Domain knowledge is incorporated into the classifier using information about affinities between words and classes: the user selects one word that correlates with the positive class, and one word correlating with the negative class. 

This is similar in spirit to the 
generalized expectation feature-labeling (GE-FL) approaches proposed by Druck et al \cite{Druck08features}. In this work, the authors use  what they call ``labeled features''. Similar to our framework, labeled features encode knowledge such as ``the word puck is a strong indicator of hockey''.

\begin{table*}[t]
	\centering
	\caption{\textbf{Text classification results.} Macro-averaged F1 score for the tasks and methods described in text. Our method (One-word), which uses one positive and one negative word with little else machinery, nears the GL-FL oracle-features method of \cite{Druck08features}, which the authors consider to be an ``upper bound" on performance their procedures can obtain. Looking at the other baselines, our method either surpasses or equals them, a surprising result since they still require relatively much more input from an oracle-like user, and use heavier machinery such as LDA.}
    \label{table:oneword}
	\begin{tabular}{|c|cccc|}
		\hline	
		{\bf Method} &{\bf med-space} &{\bf pc-mac} &{\bf baseball-hockey}  &{\bf movie}\\
		\hline
		 \textbf{One-word} ($v^+$, $v^-$) & 0.934 & 0.832 & 0.92  & 0.758 \\
		 One-word ($v^+$ only -- step 1) & 0.865 & 0.703 & 0.85  & 0.68 \\
	     GE-FL oracle-features (upper bound) & 0.952 & 0.855 & 0.954  & 0.797 \\
		 GE-FL LDA-features & 0.927 & 0.817 & 0.915 & 0.623\\
		 feat.voting (LDA)  & 0.857 & 0.740 & 0.779  & 0.616 \\
		feat. labeling (LDA) & 0.862 & 0.817 & 0.840   & 0.608\\
		 GE-FL labeled only (LDA) & 0.867 & 0.762 & 0.853 & 0.607\\	\hline
	\end{tabular}
\end{table*}

GE-FL uses labeled features given by a user to constrain
predictions on unlabeled instances, with soft constraints incorporated into the parameter estimation objective of probabilistic classifiers, penalizing predictions that yield class distributions far (in terms of KL-divergence) from reference distributions estimated using the labeled features.

The authors report results for two mechanisms to select candidate features for labeling\cite{Druck08features}:
\begin{itemize}
	\item \textbf{Oracle-features:} To obtain an upper bound, this scheme assumes an oracle provides the real label of each feature, and then features are selected according to mutual information with the class label.
	\item \textbf{LDA-features:} Alternatively, the Latent Dirichlet Allocation (LDA) topic model is applied to the data, and for each topic $t_i$, features are sorted by their probability under $t_i$ and the top features from each topic are taken.
	\item  For both candidate-generation approaches, final feature labels are chosen by assuming an oracle can provide a real label, or decide not to provide a label (such as for the word ``the"). This is simulated by computing mutual information with the class label. 
\end{itemize}

In addition to GE-FL, \cite{Druck08features} supplies performance scores for the following baselines:

\begin{itemize}
	\item \textbf{Feature voting}: Feature labels are used to vote on the
	 classification, where the occurrence of a feature (unigram) in an instance contributes a vote.
	\item \textbf{Feature labeling}: Feature labels are used to vote on
	 labels for the unlabeled instances and train a supervised
	 model with hard class assignments.
	\item \textbf{Labeled only}: GE is used to match reference distributions
	estimated from the labeled features, but unlabeled features are not used in the model.
    \item Finally, the authors also compare to supervised methods, measuring the number of labeled instances required to match their performance. We refer the reader to \cite{Druck08features} for exact figures.
\end{itemize}

In the following, we compare our algorithm to all these baselines.







%and to several baselines,  with results reported by the authors for the following data sets:
\xhdr{Experiment}
For each of the $4$ binary classification tasks described below, we split data into train and test sets. For the three  \textbf{20 newsgroups} tasks, we use built-in splits provided in python package scikit-learn \cite{Pedregosa2011sklearn}. For the \textbf{movie} data set, we run $10$ train-test ($0.90/0.10$) splits and report average results. For comparability to \cite{Druck08features}, we too use the macro-averaged F1 score, calculated using built-in functions from scikit-learn on the test set. 

For our algorithm, we tried various choices of $v^+$ and $v^-$. For the results appearing in Table \ref{table:oneword}, the following words are given as input: 
\begin{itemize}
	\item \textbf{med-space}: $v^+ = $ ``medical", $v^- = $ ``space"
	\item \textbf{pc(ibm)-mac}: $v^+ = $ ``pc", $v^- = $ ``apple"
	\item \textbf{baseball-hockey}: $v^+ = $ ``baseball", $v^- = $ ``hockey"
	\item \textbf{movie}: $v^+ = $ ``great", $v^- = $ ``stupid"
\end{itemize}

Below, we show results for different choices. Results typically did not vary widely, though there is certainly room for making the process more robust (see Section \ref{sec:criticism}). Figure \ref{fig:topwords} illustrates top words before and after selecting $v^-$. 

In the movie data set, we ran $10$ train-test splits with relatively little data. $v^- = $ ``stupid" repeatedly came up high on the negative list and was thus selected. Another top negative word was $v^- = $ ``worst", leading to similar results. 

For all experiments we fixed $C_\mathcal{P}$ to $10^{-1}$. Results were not sensitive to this choice. Finally, to solve (\ref{eq:prob1}) we used standard solvers (ECOS, SCS) with CVXPY \cite{cvxpy}.


\xhdr{Results} Table \ref{table:oneword} shows the macro-averaged F1 score for the tasks described above. The leading method in terms of raw accuracy is GL-FL with oracle-features. Note that in oracle-features, an oracle provides the real label of each feature. In other words, the algorithm has \textbf{significantly} more information than our algorithm.
Indeed, this baseline was meant to provide an ``upper bound'' the procedures of \cite{Druck08features} could give, and not as a realistic baseline. 

Our method, using as input from the user (or oracle) just one or two words, achieves a close second-best score to the oracle-features baseline on all tasks. Our method surpasses GL-FL with LDA-features and all other baselines, at times by a large margin. On the \textbf{movie} data set, we achieve a score of 0.758, compared to 0.623 or below for the non-oracle methods. Note that this is especially surprising since our method requires far less input from the user, as well as uses much simpler, lightweight techniques. 

\textbf{Runtime}. Our algorithm is very lightweight. For all $3$ \textbf{20newsgroups} tasks, runtime of Algorithm \ref{alg:One-word} was about 0.2-0.3 seconds on a standard laptop. For the \textbf{movie} task, running Algorithm \ref{alg:One-word} took about 0.45 seconds.

\subsubsection{Robustness}
We examine the robustness of our approach to choice of words, taking features chosen in real-life user experiments conducted by \cite{Druck08features}, and comparing our algorithm to a  naive baseline. In this baseline, documents containing $v^+$ are labeled positive, and documents containing $v^-$ and not $v^+$ are labeled negative.
Some word choices such as category names provide surprisingly good baselines for some of the tasks. However, many other choices of  $v^+$ and $v^-$ made by human users, fail badly with this naive method. Our model, however, remains fairly stable. The following list shows comparisons across multiple choices of $v^+,v^-$. The numbers in parentheses are results for the naive model, and the ones without parentheses are ours. 

\begin{table*}[t]
	\centering
	\caption{\textbf{Geo-tagged tweets.} For each set of geographic constraints, we show some of the top positive and negative words resulting from running our method.}
    \label{table:tweets}
	\begin{tabular}{|p{3cm}p{2.5cm}|p{5cm}|p{5cm}|}
		\hline	
	{\bf Constraints}	&  &{\bf Positive terms} &{\bf Negative terms} \\
		\hline
        \begin{minipage}{3cm}{\  \\ \includegraphics[width=3cm]{map1}} \\ \end{minipage} & \textbf{French vs. English:} Quebec > Texas  & je, est, et, le, pour &   Houston, Texas, dallas, bro, tryna, boo
		\\ \hline
		\begin{minipage}{3cm}{\  \\ \ \\ \includegraphics[width=3cm]{map3}} \\ \end{minipage} & \textbf{East Coast > West Coast:} CA > NY, CA > PA, WA > NY, WA > PA  & hella, coo, fasho,  af, la,cali, san, washington &  deadass, niggas,skool, wassup, dis, dat, philly, crib, lml, nah, dey, den \\ \hline
		\begin{minipage}{3cm}{\  \\ \ \\ \includegraphics[width=3cm]{map2}} \\ \end{minipage} & \textbf{Ranking by religiosity:} Alabama > Florida > New York & glad,thank,easter,pray, amazing,road,trip,drove, loving, relationship, spring, folks, happy, dreams, laugh, friend & mad,bitches,neva, dis, dat, niggas,ova, spanish, girls,crazy,party,fun, high, dead \\
		\hline 
	\end{tabular}
\end{table*}


\begin{itemize}
\item \textbf{med-space.} blood, space: 0.92 (0.26). cancer, space: 0.92 (0.17). medical, nasa: 0.916 (0.717). medical, sky: 0.867 (0.867). medical, moon: 0.924 (0.906). medical, earth: 0.93 (0.89). medical, mars: 0.86 (0.76).

\item \textbf{pc(ibm)-mac.} ibm, apple: 0.82 (0.54). ibm, mac: 0.79 (0.19). hp, apple: 0.77 (0.36). hp, mac 0.67 (0.08). pc, mac: 0.85 (0.52).

\item \textbf{baseball-hockey.}  braves, hockey: 0.878 (0.36). pitching, hockey: 0.913 (0.62). cubs, hockey: 0.74 (0.13). runs, hockey: 0.9 (0.82). hitter,hockey: 0.915 (0.57). jays, hockey: 0.905 (0.24). jays, nhl: 0.91 (0.36). hit, hockey: 0.92 (0.84). ball, goal: 0.915 (0.795). baseball, nhl: 0.907 (0.85); baseball, ca: 0.87 (0.36).




\end{itemize}
%\dnote{ table comparing to Druck and his baselines in the three 20newsgroups binary tasks, and to movie data set. distinguish between lda-features and oracle features. explain in body what each ones means. discuss that he uses more info etc. Give accuracy before/after using the negative word [in body of text].}


%\dnote{
%- figure: word clouds before/after using the negative word addition.
%}







